Measurement of Leptonic Asymmetries and Top Quark Polarization in ttbar Production

We present measurements of lepton (l) angular distributions in ttbar -> W+ b W- b -> l+ nu b l- nubar bbar decays produced in ppbar collisions at a center-of-mass energy of sqrt(s)=1.96TeV, where l is an electron or muon. Using data corresponding to an integrated luminosity of 5.4fb^-1, collected with the D0 detector at the Fermilab Collider, we find that the angular distributions of l- relative to anti-protons and l+ relative to protons are in agreement with each other. Combining the two distributions and correcting for detector acceptance we obtain the forward-backward asymmetry A^l_FB = (5.8 +- 5.1(stat) +- 1.3(syst))%, compared to the standard model prediction of A^l_FB (predicted) = (4.7 +- 0.1)%. This result is further combined with the measurement based on the analysis of the l+jets final state to obtain A^l_FB = (11.8 +- 3.2)%. Furthermore, we present a first study of the top-quark polarization.

==> author_list.tex <==

\affiliation{LAFEX, Centro Brasileiro de Pesquisas F\'{i}sicas, Rio de Janeiro, Brazil}
\affiliation{Universidade do Estado do Rio de Janeiro, Rio de Janeiro, Brazil}
\affiliation{Universidade Federal do ABC, Santo Andr\'e, Brazil}
\affiliation{University of Science and Technology of China, Hefei, People's Republic of China}
\affiliation{Universidad de los Andes, Bogot\'a, Colombia}
\affiliation{Charles University, Faculty of Mathematics and Physics, Center for Particle Physics, Prague, Czech Republic}
\affiliation{Czech Technical University in Prague, Prague, Czech Republic}
\affiliation{Center for Particle Physics, Institute of Physics, Academy of Sciences of the Czech Republic, Prague, Czech Republic}
\affiliation{Universidad San Francisco de Quito, Quito, Ecuador}
\affiliation{LPC, Universit\'e Blaise Pascal, CNRS/IN2P3, Clermont, France}
\affiliation{LPSC, Universit\'e Joseph Fourier Grenoble 1, CNRS/IN2P3, Institut National Polytechnique de Grenoble, Grenoble, France}
\affiliation{CPPM, Aix-Marseille Universit\'e, CNRS/IN2P3, Marseille, France}
\affiliation{LAL, Universit\'e Paris-Sud, CNRS/IN2P3, Orsay, France}
\affiliation{LPNHE, Universit\'es Paris VI and VII, CNRS/IN2P3, Paris, France}
\affiliation{CEA, Irfu, SPP, Saclay, France}
\affiliation{IPHC, Universit\'e de Strasbourg, CNRS/IN2P3, Strasbourg, France}
\affiliation{IPNL, Universit\'e Lyon 1, CNRS/IN2P3, Villeurbanne, France and Universit\'e de Lyon, Lyon, France}
\affiliation{III. Physikalisches Institut A, RWTH Aachen University, Aachen, Germany}
\affiliation{Physikalisches Institut, Universit\"at Freiburg, Freiburg, Germany}
\affiliation{II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen, G\"ottingen, Germany}
\affiliation{Institut f\"ur Physik, Universit\"at Mainz, Mainz, Germany}
\affiliation{Ludwig-Maximilians-Universit\"at M\"unchen, M\"unchen, Germany}
\affiliation{Fachbereich Physik, Bergische Universit\"at Wuppertal, Wuppertal, Germany}
\affiliation{Panjab University, Chandigarh, India}
\affiliation{Delhi University, Delhi, India}
\affiliation{Tata Institute of Fundamental Research, Mumbai, India}
\affiliation{University College Dublin, Dublin, Ireland}
\affiliation{Korea Detector Laboratory, Korea University, Seoul, Korea}
\affiliation{CINVESTAV, Mexico City, Mexico}
\affiliation{Nikhef, Science Park, Amsterdam, the Netherlands}
\affiliation{Radboud University Nijmegen, Nijmegen, the Netherlands}
\affiliation{Joint Institute for Nuclear Research, Dubna, Russia}
\affiliation{Institute for Theoretical and Experimental Physics, Moscow, Russia}
\affiliation{Moscow State University, Moscow, Russia}
\affiliation{Institute for High Energy Physics, Protvino, Russia}
\affiliation{Petersburg Nuclear Physics Institute, St. Petersburg, Russia}
\affiliation{Instituci\'{o} Catalana de Recerca i Estudis Avan\c{c}ats (ICREA) and Institut de F\'{i}sica d'Altes Energies (IFAE), Barcelona, Spain}
\affiliation{Uppsala University, Uppsala, Sweden}
\affiliation{Lancaster University, Lancaster LA1 4YB, United Kingdom}
\affiliation{Imperial College London, London SW7 2AZ, United Kingdom}
\affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\affiliation{University of Arizona, Tucson, Arizona 85721, USA}
\affiliation{University of California Riverside, Riverside, California 92521, USA}
\affiliation{Florida State University, Tallahassee, Florida 32306, USA}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607, USA}
\affiliation{Northern Illinois University, DeKalb, Illinois 60115, USA}
\affiliation{Northwestern University, Evanston, Illinois 60208, USA}
\affiliation{Indiana University, Bloomington, Indiana 47405, USA}
\affiliation{Purdue University Calumet, Hammond, Indiana 46323, USA}
\affiliation{University of Notre Dame, Notre Dame, Indiana 46556, USA}
\affiliation{Iowa State University, Ames, Iowa 50011, USA}
\affiliation{University of Kansas, Lawrence, Kansas 66045, USA}
\affiliation{Kansas State University, Manhattan, Kansas 66506, USA}
\affiliation{Louisiana Tech University, Ruston, Louisiana 71272, USA}
\affiliation{Boston University, Boston, Massachusetts 02215, USA}
\affiliation{Northeastern University, Boston, Massachusetts 02115, USA}
\affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\affiliation{University of Mississippi, University, Mississippi 38677, USA}
\affiliation{University of Nebraska, Lincoln, Nebraska 68588, USA}
\affiliation{Rutgers University, Piscataway, New Jersey 08855, USA}
\affiliation{Princeton University, Princeton, New Jersey 08544, USA}
\affiliation{State University of New York, Buffalo, New York 14260, USA}
\affiliation{University of Rochester, Rochester, New York 14627, USA}
\affiliation{State University of New York, Stony Brook, New York 11794, USA}
\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\affiliation{Langston University, Langston, Oklahoma 73050, USA}
\affiliation{University of Oklahoma, Norman, Oklahoma 73019, USA}
\affiliation{Oklahoma State University, Stillwater, Oklahoma 74078, USA}
\affiliation{Brown University, Providence, Rhode Island 02912, USA}
\affiliation{University of Texas, Arlington, Texas 76019, USA}
\affiliation{Southern Methodist University, Dallas, Texas 75275, USA}
\affiliation{Rice University, Houston, Texas 77005, USA}
\affiliation{University of Virginia, Charlottesville, Virginia 22901, USA}
\affiliation{University of Washington, Seattle, Washington 98195, USA}
%
\author{V.M.~Abazov} \affiliation{Joint Institute for Nuclear Research, Dubna, Russia}
\author{B.~Abbott} \affiliation{University of Oklahoma, Norman, Oklahoma 73019, USA}
\author{B.S.~Acharya} \affiliation{Tata Institute of Fundamental Research, Mumbai, India}
\author{M.~Adams} \affiliation{University of Illinois at Chicago, Chicago, Illinois 60607, USA}
\author{T.~Adams} \affiliation{Florida State University, Tallahassee, Florida 32306, USA}
\author{G.D.~Alexeev} \affiliation{Joint Institute for Nuclear Research, Dubna, Russia}
\author{G.~Alkhazov} \affiliation{Petersburg Nuclear Physics Institute, St. Petersburg, Russia}
\author{A.~Alton$^{a}$} \affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\author{G.~Alverson} \affiliation{Northeastern University, Boston, Massachusetts 02115, USA}
\author{A.~Askew} \affiliation{Florida State University, Tallahassee, Florida 32306, USA}
\author{S.~Atkins} \affiliation{Louisiana Tech University, Ruston, Louisiana 71272, USA}
\author{K.~Augsten} \affiliation{Czech Technical University in Prague, Prague, Czech Republic}
\author{C.~Avila} \affiliation{Universidad de los Andes, Bogot\'a, Colombia}
\author{F.~Badaud} \affiliation{LPC, Universit\'e Blaise Pascal, CNRS/IN2P3, Clermont, France}
\author{L.~Bagby} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{B.~Baldin} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{D.V.~Bandurin} \affiliation{Florida State University, Tallahassee, Florida 32306, USA}
\author{S.~Banerjee} \affiliation{Tata Institute of Fundamental Research, Mumbai, India}
\author{E.~Barberis} \affiliation{Northeastern University, Boston, Massachusetts 02115, USA}
\author{P.~Baringer} \affiliation{University of Kansas, Lawrence, Kansas 66045, USA}
\author{J.F.~Bartlett} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{U.~Bassler} \affiliation{CEA, Irfu, SPP, Saclay, France}
\author{V.~Bazterra} \affiliation{University of Illinois at Chicago, Chicago, Illinois 60607, USA}
\author{A.~Bean} \affiliation{University of Kansas, Lawrence, Kansas 66045, USA}
\author{M.~Begalli} \affiliation{Universidade do Estado do Rio de Janeiro, Rio de Janeiro, Brazil}
\author{L.~Bellantoni} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{S.B.~Beri} \affiliation{Panjab University, Chandigarh, India}
\author{G.~Bernardi} \affiliation{LPNHE, Universit\'es Paris VI and VII, CNRS/IN2P3, Paris, France}
\author{R.~Bernhard} \affiliation{Physikalisches Institut, Universit\"at Freiburg, Freiburg, Germany}
\author{I.~Bertram} \affiliation{Lancaster University, Lancaster LA1 4YB, United Kingdom}
\author{M.~Besan\c{c}on} \affiliation{CEA, Irfu, SPP, Saclay, France}
\author{R.~Beuselinck} \affiliation{Imperial College London, London SW7 2AZ, United Kingdom}
\author{P.C.~Bhat} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{S.~Bhatia} \affiliation{University of Mississippi, University, Mississippi 38677, USA}
\author{V.~Bhatnagar} \affiliation{Panjab University, Chandigarh, India}
\author{G.~Blazey} \affiliation{Northern Illinois University, DeKalb, Illinois 60115, USA}
\author{S.~Blessing} \affiliation{Florida State University, Tallahassee, Florida 32306, USA}
\author{K.~Bloom} \affiliation{University of Nebraska, Lincoln, Nebraska 68588, USA}
\author{A.~Boehnlein} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{D.~Boline} \affiliation{State University of New York, Stony Brook, New York 11794, USA}
\author{E.E.~Boos} \affiliation{Moscow State University, Moscow, Russia}
\author{G.~Borissov} \affiliation{Lancaster University, Lancaster LA1 4YB, United Kingdom}
\author{T.~Bose} \affiliation{Boston University, Boston, Massachusetts 02215, USA}
\author{A.~Brandt} \affiliation{University of Texas, Arlington, Texas 76019, USA}
\author{O.~Brandt} \affiliation{II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen, G\"ottingen, Germany}
\author{R.~Brock} \affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{A.~Bross} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{D.~Brown} \affiliation{LPNHE, Universit\'es Paris VI and VII, CNRS/IN2P3, Paris, France}
\author{J.~Brown} \affiliation{LPNHE, Universit\'es Paris VI and VII, CNRS/IN2P3, Paris, France}
\author{X.B.~Bu} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.~Buehler} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{V.~Buescher} \affiliation{Institut f\"ur Physik, Universit\"at Mainz, Mainz, Germany}
\author{V.~Bunichev} \affiliation{Moscow State University, Moscow, Russia}
\author{S.~Burdin$^{b}$} \affiliation{Lancaster University, Lancaster LA1 4YB, United Kingdom}
\author{C.P.~Buszello} \affiliation{Uppsala University, Uppsala, Sweden}
\author{E.~Camacho-P\'erez} \affiliation{CINVESTAV, Mexico City, Mexico}
\author{B.C.K.~Casey} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{H.~Castilla-Valdez} \affiliation{CINVESTAV, Mexico City, Mexico}
\author{S.~Caughron} \affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{S.~Chakrabarti} \affiliation{State University of New York, Stony Brook, New York 11794, USA}
\author{D.~Chakraborty} \affiliation{Northern Illinois University, DeKalb, Illinois 60115, USA}
\author{K.M.~Chan} \affiliation{University of Notre Dame, Notre Dame, Indiana 46556, USA}
\author{A.~Chandra} \affiliation{Rice University, Houston, Texas 77005, USA}
\author{E.~Chapon} \affiliation{CEA, Irfu, SPP, Saclay, France}
\author{G.~Chen} \affiliation{University of Kansas, Lawrence, Kansas 66045, USA}
\author{S.~Chevalier-Th\'ery} \affiliation{CEA, Irfu, SPP, Saclay, France}
\author{D.K.~Cho} \affiliation{Brown University, Providence, Rhode Island 02912, USA}
\author{S.W.~Cho} \affiliation{Korea Detector Laboratory, Korea University, Seoul, Korea}
\author{S.~Choi} \affiliation{Korea Detector Laboratory, Korea University, Seoul, Korea}
\author{B.~Choudhary} \affiliation{Delhi University, Delhi, India}
\author{S.~Cihangir} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{D.~Claes} \affiliation{University of Nebraska, Lincoln, Nebraska 68588, USA}
\author{J.~Clutter} \affiliation{University of Kansas, Lawrence, Kansas 66045, USA}
\author{M.~Cooke} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{W.E.~Cooper} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.~Corcoran} \affiliation{Rice University, Houston, Texas 77005, USA}
\author{F.~Couderc} \affiliation{CEA, Irfu, SPP, Saclay, France}
\author{M.-C.~Cousinou} \affiliation{CPPM, Aix-Marseille Universit\'e, CNRS/IN2P3, Marseille, France}
\author{A.~Croc} \affiliation{CEA, Irfu, SPP, Saclay, France}
\author{D.~Cutts} \affiliation{Brown University, Providence, Rhode Island 02912, USA}
\author{A.~Das} \affiliation{University of Arizona, Tucson, Arizona 85721, USA}
\author{G.~Davies} \affiliation{Imperial College London, London SW7 2AZ, United Kingdom}
\author{S.J.~de~Jong} \affiliation{Nikhef, Science Park, Amsterdam, the Netherlands} \affiliation{Radboud University Nijmegen, Nijmegen, the Netherlands}
\author{E.~De~La~Cruz-Burelo} \affiliation{CINVESTAV, Mexico City, Mexico}
\author{F.~D\'eliot} \affiliation{CEA, Irfu, SPP, Saclay, France}
\author{R.~Demina} \affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{D.~Denisov} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{S.P.~Denisov} \affiliation{Institute for High Energy Physics, Protvino, Russia}
\author{S.~Desai} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{C.~Deterre} \affiliation{CEA, Irfu, SPP, Saclay, France}
\author{K.~DeVaughan} \affiliation{University of Nebraska, Lincoln, Nebraska 68588, USA}
\author{H.T.~Diehl} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.~Diesburg} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{P.F.~Ding} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{A.~Dominguez} \affiliation{University of Nebraska, Lincoln, Nebraska 68588, USA}
\author{A.~Dubey} \affiliation{Delhi University, Delhi, India}
\author{L.V.~Dudko} \affiliation{Moscow State University, Moscow, Russia}
\author{D.~Duggan} \affiliation{Rutgers University, Piscataway, New Jersey 08855, USA}
\author{A.~Duperrin} \affiliation{CPPM, Aix-Marseille Universit\'e, CNRS/IN2P3, Marseille, France}
\author{S.~Dutt} \affiliation{Panjab University, Chandigarh, India}
\author{A.~Dyshkant} \affiliation{Northern Illinois University, DeKalb, Illinois 60115, USA}
\author{M.~Eads} \affiliation{University of Nebraska, Lincoln, Nebraska 68588, USA}
\author{D.~Edmunds} \affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{J.~Ellison} \affiliation{University of California Riverside, Riverside, California 92521, USA}
\author{V.D.~Elvira} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{Y.~Enari} \affiliation{LPNHE, Universit\'es Paris VI and VII, CNRS/IN2P3, Paris, France}
\author{H.~Evans} \affiliation{Indiana University, Bloomington, Indiana 47405, USA}
\author{A.~Evdokimov} \affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{V.N.~Evdokimov} \affiliation{Institute for High Energy Physics, Protvino, Russia}
\author{G.~Facini} \affiliation{Northeastern University, Boston, Massachusetts 02115, USA}
\author{L.~Feng} \affiliation{Northern Illinois University, DeKalb, Illinois 60115, USA}
\author{T.~Ferbel} \affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{F.~Fiedler} \affiliation{Institut f\"ur Physik, Universit\"at Mainz, Mainz, Germany}
\author{F.~Filthaut} \affiliation{Nikhef, Science Park, Amsterdam, the Netherlands} \affiliation{Radboud University Nijmegen, Nijmegen, the Netherlands}
\author{W.~Fisher} \affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{H.E.~Fisk} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.~Fortner} \affiliation{Northern Illinois University, DeKalb, Illinois 60115, USA}
\author{H.~Fox} \affiliation{Lancaster University, Lancaster LA1 4YB, United Kingdom}
\author{S.~Fuess} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{A.~Garcia-Bellido} \affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{J.A.~Garc\'{\i}a-Gonz\'alez} \affiliation{CINVESTAV, Mexico City, Mexico}
\author{G.A.~Garc\'ia-Guerra$^{c}$} \affiliation{CINVESTAV, Mexico City, Mexico}
\author{V.~Gavrilov} \affiliation{Institute for Theoretical and Experimental Physics, Moscow, Russia}
\author{P.~Gay} \affiliation{LPC, Universit\'e Blaise Pascal, CNRS/IN2P3, Clermont, France}
\author{W.~Geng} \affiliation{CPPM, Aix-Marseille Universit\'e, CNRS/IN2P3, Marseille, France} \affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{D.~Gerbaudo} \affiliation{Princeton University, Princeton, New Jersey 08544, USA}
\author{C.E.~Gerber} \affiliation{University of Illinois at Chicago, Chicago, Illinois 60607, USA}
\author{Y.~Gershtein} \affiliation{Rutgers University, Piscataway, New Jersey 08855, USA}
\author{G.~Ginther} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA} \affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{G.~Golovanov} \affiliation{Joint Institute for Nuclear Research, Dubna, Russia}
\author{A.~Goussiou} \affiliation{University of Washington, Seattle, Washington 98195, USA}
\author{P.D.~Grannis} \affiliation{State University of New York, Stony Brook, New York 11794, USA}
\author{S.~Greder} \affiliation{IPHC, Universit\'e de Strasbourg, CNRS/IN2P3, Strasbourg, France}
\author{H.~Greenlee} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{G.~Grenier} \affiliation{IPNL, Universit\'e Lyon 1, CNRS/IN2P3, Villeurbanne, France and Universit\'e de Lyon, Lyon, France}
\author{Ph.~Gris} \affiliation{LPC, Universit\'e Blaise Pascal, CNRS/IN2P3, Clermont, France}
\author{J.-F.~Grivaz} \affiliation{LAL, Universit\'e Paris-Sud, CNRS/IN2P3, Orsay, France}
\author{A.~Grohsjean$^{d}$} \affiliation{CEA, Irfu, SPP, Saclay, France}
\author{S.~Gr\"unendahl} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.W.~Gr{\"u}newald} \affiliation{University College Dublin, Dublin, Ireland}
\author{T.~Guillemin} \affiliation{LAL, Universit\'e Paris-Sud, CNRS/IN2P3, Orsay, France}
\author{G.~Gutierrez} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{P.~Gutierrez} \affiliation{University of Oklahoma, Norman, Oklahoma 73019, USA}
\author{S.~Hagopian} \affiliation{Florida State University, Tallahassee, Florida 32306, USA}
\author{J.~Haley} \affiliation{Northeastern University, Boston, Massachusetts 02115, USA}
\author{L.~Han} \affiliation{University of Science and Technology of China, Hefei, People's Republic of China}
\author{K.~Harder} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{A.~Harel} \affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{J.M.~Hauptman} \affiliation{Iowa State University, Ames, Iowa 50011, USA}
\author{J.~Hays} \affiliation{Imperial College London, London SW7 2AZ, United Kingdom}
\author{T.~Head} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{T.~Hebbeker} \affiliation{III. Physikalisches Institut A, RWTH Aachen University, Aachen, Germany}
\author{D.~Hedin} \affiliation{Northern Illinois University, DeKalb, Illinois 60115, USA}
\author{H.~Hegab} \affiliation{Oklahoma State University, Stillwater, Oklahoma 74078, USA}
\author{A.P.~Heinson} \affiliation{University of California Riverside, Riverside, California 92521, USA}
\author{U.~Heintz} \affiliation{Brown University, Providence, Rhode Island 02912, USA}
\author{C.~Hensel} \affiliation{II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen, G\"ottingen, Germany}
\author{I.~Heredia-De~La~Cruz} \affiliation{CINVESTAV, Mexico City, Mexico}
\author{K.~Herner} \affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\author{G.~Hesketh$^{f}$} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{M.D.~Hildreth} \affiliation{University of Notre Dame, Notre Dame, Indiana 46556, USA}
\author{R.~Hirosky} \affiliation{University of Virginia, Charlottesville, Virginia 22901, USA}
\author{T.~Hoang} \affiliation{Florida State University, Tallahassee, Florida 32306, USA}
\author{J.D.~Hobbs} \affiliation{State University of New York, Stony Brook, New York 11794, USA}
\author{B.~Hoeneisen} \affiliation{Universidad San Francisco de Quito, Quito, Ecuador}
\author{J.~Hogan} \affiliation{Rice University, Houston, Texas 77005, USA}
\author{M.~Hohlfeld} \affiliation{Institut f\"ur Physik, Universit\"at Mainz, Mainz, Germany}
\author{I.~Howley} \affiliation{University of Texas, Arlington, Texas 76019, USA}
\author{Z.~Hubacek} \affiliation{Czech Technical University in Prague, Prague, Czech Republic} \affiliation{CEA, Irfu, SPP, Saclay, France}
\author{V.~Hynek} \affiliation{Czech Technical University in Prague, Prague, Czech Republic}
\author{I.~Iashvili} \affiliation{State University of New York, Buffalo, New York 14260, USA}
\author{Y.~Ilchenko} \affiliation{Southern Methodist University, Dallas, Texas 75275, USA}
\author{R.~Illingworth} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{A.S.~Ito} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{S.~Jabeen} \affiliation{Brown University, Providence, Rhode Island 02912, USA}
\author{M.~Jaffr\'e} \affiliation{LAL, Universit\'e Paris-Sud, CNRS/IN2P3, Orsay, France}
\author{A.~Jayasinghe} \affiliation{University of Oklahoma, Norman, Oklahoma 73019, USA}
\author{M.S.~Jeong} \affiliation{Korea Detector Laboratory, Korea University, Seoul, Korea}
\author{R.~Jesik} \affiliation{Imperial College London, London SW7 2AZ, United Kingdom}
\author{K.~Johns} \affiliation{University of Arizona, Tucson, Arizona 85721, USA}
\author{E.~Johnson} \affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{M.~Johnson} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{A.~Jonckheere} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{P.~Jonsson} \affiliation{Imperial College London, London SW7 2AZ, United Kingdom}
\author{J.~Joshi} \affiliation{University of California Riverside, Riverside, California 92521, USA}
\author{A.W.~Jung} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{A.~Juste} \affiliation{Instituci\'{o} Catalana de Recerca i Estudis Avan\c{c}ats (ICREA) and Institut de F\'{i}sica d'Altes Energies (IFAE), Barcelona, Spain}
\author{K.~Kaadze} \affiliation{Kansas State University, Manhattan, Kansas 66506, USA}
\author{E.~Kajfasz} \affiliation{CPPM, Aix-Marseille Universit\'e, CNRS/IN2P3, Marseille, France}
\author{D.~Karmanov} \affiliation{Moscow State University, Moscow, Russia}
\author{P.A.~Kasper} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{I.~Katsanos} \affiliation{University of Nebraska, Lincoln, Nebraska 68588, USA}
\author{R.~Kehoe} \affiliation{Southern Methodist University, Dallas, Texas 75275, USA}
\author{S.~Kermiche} \affiliation{CPPM, Aix-Marseille Universit\'e, CNRS/IN2P3, Marseille, France}
\author{N.~Khalatyan} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{A.~Khanov} \affiliation{Oklahoma State University, Stillwater, Oklahoma 74078, USA}
\author{A.~Kharchilava} \affiliation{State University of New York, Buffalo, New York 14260, USA}
\author{Y.N.~Kharzheev} \affiliation{Joint Institute for Nuclear Research, Dubna, Russia}
\author{I.~Kiselevich} \affiliation{Institute for Theoretical and Experimental Physics, Moscow, Russia}
\author{J.M.~Kohli} \affiliation{Panjab University, Chandigarh, India}
\author{A.V.~Kozelov} \affiliation{Institute for High Energy Physics, Protvino, Russia}
\author{J.~Kraus} \affiliation{University of Mississippi, University, Mississippi 38677, USA}
\author{S.~Kulikov} \affiliation{Institute for High Energy Physics, Protvino, Russia}
\author{A.~Kumar} \affiliation{State University of New York, Buffalo, New York 14260, USA}
\author{A.~Kupco} \affiliation{Center for Particle Physics, Institute of Physics, Academy of Sciences of the Czech Republic, Prague, Czech Republic}
\author{T.~Kur\v{c}a} \affiliation{IPNL, Universit\'e Lyon 1, CNRS/IN2P3, Villeurbanne, France and Universit\'e de Lyon, Lyon, France}
\author{V.A.~Kuzmin} \affiliation{Moscow State University, Moscow, Russia}
\author{S.~Lammers} \affiliation{Indiana University, Bloomington, Indiana 47405, USA}
\author{G.~Landsberg} \affiliation{Brown University, Providence, Rhode Island 02912, USA}
\author{P.~Lebrun} \affiliation{IPNL, Universit\'e Lyon 1, CNRS/IN2P3, Villeurbanne, France and Universit\'e de Lyon, Lyon, France}
\author{H.S.~Lee} \affiliation{Korea Detector Laboratory, Korea University, Seoul, Korea}
\author{S.W.~Lee} \affiliation{Iowa State University, Ames, Iowa 50011, USA}
\author{W.M.~Lee} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{X.~Lei} \affiliation{University of Arizona, Tucson, Arizona 85721, USA}
\author{J.~Lellouch} \affiliation{LPNHE, Universit\'es Paris VI and VII, CNRS/IN2P3, Paris, France}
\author{H.~Li} \affiliation{LPSC, Universit\'e Joseph Fourier Grenoble 1, CNRS/IN2P3, Institut National Polytechnique de Grenoble, Grenoble, France}
\author{L.~Li} \affiliation{University of California Riverside, Riverside, California 92521, USA}
\author{Q.Z.~Li} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{J.K.~Lim} \affiliation{Korea Detector Laboratory, Korea University, Seoul, Korea}
\author{D.~Lincoln} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{J.~Linnemann} \affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{V.V.~Lipaev} \affiliation{Institute for High Energy Physics, Protvino, Russia}
\author{R.~Lipton} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{H.~Liu} \affiliation{Southern Methodist University, Dallas, Texas 75275, USA}
\author{Y.~Liu} \affiliation{University of Science and Technology of China, Hefei, People's Republic of China}
\author{A.~Lobodenko} \affiliation{Petersburg Nuclear Physics Institute, St. Petersburg, Russia}
\author{M.~Lokajicek} \affiliation{Center for Particle Physics, Institute of Physics, Academy of Sciences of the Czech Republic, Prague, Czech Republic}
\author{R.~Lopes~de~Sa} \affiliation{State University of New York, Stony Brook, New York 11794, USA}
\author{H.J.~Lubatti} \affiliation{University of Washington, Seattle, Washington 98195, USA}
\author{R.~Luna-Garcia$^{g}$} \affiliation{CINVESTAV, Mexico City, Mexico}
\author{A.L.~Lyon} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{A.K.A.~Maciel} \affiliation{LAFEX, Centro Brasileiro de Pesquisas F\'{i}sicas, Rio de Janeiro, Brazil}
\author{R.~Madar} \affiliation{CEA, Irfu, SPP, Saclay, France}
\author{R.~Maga\~na-Villalba} \affiliation{CINVESTAV, Mexico City, Mexico}
\author{S.~Malik} \affiliation{University of Nebraska, Lincoln, Nebraska 68588, USA}
\author{V.L.~Malyshev} \affiliation{Joint Institute for Nuclear Research, Dubna, Russia}
\author{Y.~Maravin} \affiliation{Kansas State University, Manhattan, Kansas 66506, USA}
\author{J.~Mart\'{\i}nez-Ortega} \affiliation{CINVESTAV, Mexico City, Mexico}
\author{R.~McCarthy} \affiliation{State University of New York, Stony Brook, New York 11794, USA}
\author{C.L.~McGivern} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{M.M.~Meijer} \affiliation{Nikhef, Science Park, Amsterdam, the Netherlands} \affiliation{Radboud University Nijmegen, Nijmegen, the Netherlands}
\author{A.~Melnitchouk} \affiliation{University of Mississippi, University, Mississippi 38677, USA}
\author{D.~Menezes} \affiliation{Northern Illinois University, DeKalb, Illinois 60115, USA}
\author{P.G.~Mercadante} \affiliation{Universidade Federal do ABC, Santo Andr\'e, Brazil}
\author{M.~Merkin} \affiliation{Moscow State University, Moscow, Russia}
\author{A.~Meyer} \affiliation{III. Physikalisches Institut A, RWTH Aachen University, Aachen, Germany}
\author{J.~Meyer} \affiliation{II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen, G\"ottingen, Germany}
\author{F.~Miconi} \affiliation{IPHC, Universit\'e de Strasbourg, CNRS/IN2P3, Strasbourg, France}
\author{N.K.~Mondal} \affiliation{Tata Institute of Fundamental Research, Mumbai, India}
\author{M.~Mulhearn} \affiliation{University of Virginia, Charlottesville, Virginia 22901, USA}
\author{E.~Nagy} \affiliation{CPPM, Aix-Marseille Universit\'e, CNRS/IN2P3, Marseille, France}
\author{M.~Naimuddin} \affiliation{Delhi University, Delhi, India}
\author{M.~Narain} \affiliation{Brown University, Providence, Rhode Island 02912, USA}
\author{R.~Nayyar} \affiliation{University of Arizona, Tucson, Arizona 85721, USA}
\author{H.A.~Neal} \affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\author{J.P.~Negret} \affiliation{Universidad de los Andes, Bogot\'a, Colombia}
\author{P.~Neustroev} \affiliation{Petersburg Nuclear Physics Institute, St. Petersburg, Russia}
\author{T.~Nunnemann} \affiliation{Ludwig-Maximilians-Universit\"at M\"unchen, M\"unchen, Germany}
\author{D.~Orbaker} \affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{J.~Orduna} \affiliation{Rice University, Houston, Texas 77005, USA}
\author{N.~Osman} \affiliation{CPPM, Aix-Marseille Universit\'e, CNRS/IN2P3, Marseille, France}
\author{J.~Osta} \affiliation{University of Notre Dame, Notre Dame, Indiana 46556, USA}
\author{M.~Padilla} \affiliation{University of California Riverside, Riverside, California 92521, USA}
\author{A.~Pal} \affiliation{University of Texas, Arlington, Texas 76019, USA}
\author{N.~Parashar} \affiliation{Purdue University Calumet, Hammond, Indiana 46323, USA}
\author{V.~Parihar} \affiliation{Brown University, Providence, Rhode Island 02912, USA}
\author{S.K.~Park} \affiliation{Korea Detector Laboratory, Korea University, Seoul, Korea}
\author{R.~Partridge$^{e}$} \affiliation{Brown University, Providence, Rhode Island 02912, USA}
\author{N.~Parua} \affiliation{Indiana University, Bloomington, Indiana 47405, USA}
\author{A.~Patwa} \affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{B.~Penning} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.~Perfilov} \affiliation{Moscow State University, Moscow, Russia}
\author{Y.~Peters} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{K.~Petridis} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{G.~Petrillo} \affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{P.~P\'etroff} \affiliation{LAL, Universit\'e Paris-Sud, CNRS/IN2P3, Orsay, France}
\author{M.-A.~Pleier} \affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{P.L.M.~Podesta-Lerma$^{h}$} \affiliation{CINVESTAV, Mexico City, Mexico}
\author{V.M.~Podstavkov} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{A.V.~Popov} \affiliation{Institute for High Energy Physics, Protvino, Russia}
\author{M.~Prewitt} \affiliation{Rice University, Houston, Texas 77005, USA}
\author{D.~Price} \affiliation{Indiana University, Bloomington, Indiana 47405, USA}
\author{N.~Prokopenko} \affiliation{Institute for High Energy Physics, Protvino, Russia}
\author{J.~Qian} \affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\author{A.~Quadt} \affiliation{II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen, G\"ottingen, Germany}
\author{B.~Quinn} \affiliation{University of Mississippi, University, Mississippi 38677, USA}
\author{M.S.~Rangel} \affiliation{LAFEX, Centro Brasileiro de Pesquisas F\'{i}sicas, Rio de Janeiro, Brazil}
\author{K.~Ranjan} \affiliation{Delhi University, Delhi, India}
\author{P.N.~Ratoff} \affiliation{Lancaster University, Lancaster LA1 4YB, United Kingdom}
\author{I.~Razumov} \affiliation{Institute for High Energy Physics, Protvino, Russia}
\author{P.~Renkel} \affiliation{Southern Methodist University, Dallas, Texas 75275, USA}
\author{I.~Ripp-Baudot} \affiliation{IPHC, Universit\'e de Strasbourg, CNRS/IN2P3, Strasbourg, France}
\author{F.~Rizatdinova} \affiliation{Oklahoma State University, Stillwater, Oklahoma 74078, USA}
\author{M.~Rominsky} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{A.~Ross} \affiliation{Lancaster University, Lancaster LA1 4YB, United Kingdom}
\author{C.~Royon} \affiliation{CEA, Irfu, SPP, Saclay, France}
\author{P.~Rubinov} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{R.~Ruchti} \affiliation{University of Notre Dame, Notre Dame, Indiana 46556, USA}
\author{G.~Sajot} \affiliation{LPSC, Universit\'e Joseph Fourier Grenoble 1, CNRS/IN2P3, Institut National Polytechnique de Grenoble, Grenoble, France}
\author{P.~Salcido} \affiliation{Northern Illinois University, DeKalb, Illinois 60115, USA}
\author{A.~S\'anchez-Hern\'andez} \affiliation{CINVESTAV, Mexico City, Mexico}
\author{M.P.~Sanders} \affiliation{Ludwig-Maximilians-Universit\"at M\"unchen, M\"unchen, Germany}
\author{A.S.~Santos$^{i}$} \affiliation{LAFEX, Centro Brasileiro de Pesquisas F\'{i}sicas, Rio de Janeiro, Brazil}
\author{G.~Savage} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{L.~Sawyer} \affiliation{Louisiana Tech University, Ruston, Louisiana 71272, USA}
\author{T.~Scanlon} \affiliation{Imperial College London, London SW7 2AZ, United Kingdom}
\author{R.D.~Schamberger} \affiliation{State University of New York, Stony Brook, New York 11794, USA}
\author{Y.~Scheglov} \affiliation{Petersburg Nuclear Physics Institute, St. Petersburg, Russia}
\author{H.~Schellman} \affiliation{Northwestern University, Evanston, Illinois 60208, USA}
\author{S.~Schlobohm} \affiliation{University of Washington, Seattle, Washington 98195, USA}
\author{C.~Schwanenberger} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{R.~Schwienhorst} \affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{J.~Sekaric} \affiliation{University of Kansas, Lawrence, Kansas 66045, USA}
\author{H.~Severini} \affiliation{University of Oklahoma, Norman, Oklahoma 73019, USA}
\author{E.~Shabalina} \affiliation{II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen, G\"ottingen, Germany}
\author{V.~Shary} \affiliation{CEA, Irfu, SPP, Saclay, France}
\author{S.~Shaw} \affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{A.A.~Shchukin} \affiliation{Institute for High Energy Physics, Protvino, Russia}
\author{R.K.~Shivpuri} \affiliation{Delhi University, Delhi, India}
\author{V.~Simak} \affiliation{Czech Technical University in Prague, Prague, Czech Republic}
\author{P.~Skubic} \affiliation{University of Oklahoma, Norman, Oklahoma 73019, USA}
\author{P.~Slattery} \affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{D.~Smirnov} \affiliation{University of Notre Dame, Notre Dame, Indiana 46556, USA}
\author{K.J.~Smith} \affiliation{State University of New York, Buffalo, New York 14260, USA}
\author{G.R.~Snow} \affiliation{University of Nebraska, Lincoln, Nebraska 68588, USA}
\author{J.~Snow} \affiliation{Langston University, Langston, Oklahoma 73050, USA}
\author{S.~Snyder} \affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{S.~S{\"o}ldner-Rembold} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{L.~Sonnenschein} \affiliation{III. Physikalisches Institut A, RWTH Aachen University, Aachen, Germany}
\author{K.~Soustruznik} \affiliation{Charles University, Faculty of Mathematics and Physics, Center for Particle Physics, Prague, Czech Republic}
\author{J.~Stark} \affiliation{LPSC, Universit\'e Joseph Fourier Grenoble 1, CNRS/IN2P3, Institut National Polytechnique de Grenoble, Grenoble, France}
\author{D.A.~Stoyanova} \affiliation{Institute for High Energy Physics, Protvino, Russia}
\author{M.~Strauss} \affiliation{University of Oklahoma, Norman, Oklahoma 73019, USA}
\author{L.~Suter} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{P.~Svoisky} \affiliation{University of Oklahoma, Norman, Oklahoma 73019, USA}
\author{M.~Takahashi} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{M.~Titov} \affiliation{CEA, Irfu, SPP, Saclay, France}
\author{V.V.~Tokmenin} \affiliation{Joint Institute for Nuclear Research, Dubna, Russia}
\author{Y.-T.~Tsai} \affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{K.~Tschann-Grimm} \affiliation{State University of New York, Stony Brook, New York 11794, USA}
\author{D.~Tsybychev} \affiliation{State University of New York, Stony Brook, New York 11794, USA}
\author{B.~Tuchming} \affiliation{CEA, Irfu, SPP, Saclay, France}
\author{C.~Tully} \affiliation{Princeton University, Princeton, New Jersey 08544, USA}
\author{L.~Uvarov} \affiliation{Petersburg Nuclear Physics Institute, St. Petersburg, Russia}
\author{S.~Uvarov} \affiliation{Petersburg Nuclear Physics Institute, St. Petersburg, Russia}
\author{S.~Uzunyan} \affiliation{Northern Illinois University, DeKalb, Illinois 60115, USA}
\author{R.~Van~Kooten} \affiliation{Indiana University, Bloomington, Indiana 47405, USA}
\author{W.M.~van~Leeuwen} \affiliation{Nikhef, Science Park, Amsterdam, the Netherlands}
\author{N.~Varelas} \affiliation{University of Illinois at Chicago, Chicago, Illinois 60607, USA}
\author{E.W.~Varnes} \affiliation{University of Arizona, Tucson, Arizona 85721, USA}
\author{I.A.~Vasilyev} \affiliation{Institute for High Energy Physics, Protvino, Russia}
\author{P.~Verdier} \affiliation{IPNL, Universit\'e Lyon 1, CNRS/IN2P3, Villeurbanne, France and Universit\'e de Lyon, Lyon, France}
\author{A.Y.~Verkheev} \affiliation{Joint Institute for Nuclear Research, Dubna, Russia}
\author{L.S.~Vertogradov} \affiliation{Joint Institute for Nuclear Research, Dubna, Russia}
\author{M.~Verzocchi} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.~Vesterinen} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{D.~Vilanova} \affiliation{CEA, Irfu, SPP, Saclay, France}
\author{P.~Vokac} \affiliation{Czech Technical University in Prague, Prague, Czech Republic}
\author{H.D.~Wahl} \affiliation{Florida State University, Tallahassee, Florida 32306, USA}
\author{M.H.L.S.~Wang} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{J.~Warchol} \affiliation{University of Notre Dame, Notre Dame, Indiana 46556, USA}
\author{G.~Watts} \affiliation{University of Washington, Seattle, Washington 98195, USA}
\author{M.~Wayne} \affiliation{University of Notre Dame, Notre Dame, Indiana 46556, USA}
\author{J.~Weichert} \affiliation{Institut f\"ur Physik, Universit\"at Mainz, Mainz, Germany}
\author{L.~Welty-Rieger} \affiliation{Northwestern University, Evanston, Illinois 60208, USA}
\author{A.~White} \affiliation{University of Texas, Arlington, Texas 76019, USA}
\author{D.~Wicke} \affiliation{Fachbereich Physik, Bergische Universit\"at Wuppertal, Wuppertal, Germany}
\author{M.R.J.~Williams} \affiliation{Lancaster University, Lancaster LA1 4YB, United Kingdom}
\author{G.W.~Wilson} \affiliation{University of Kansas, Lawrence, Kansas 66045, USA}
\author{M.~Wobisch} \affiliation{Louisiana Tech University, Ruston, Louisiana 71272, USA}
\author{D.R.~Wood} \affiliation{Northeastern University, Boston, Massachusetts 02115, USA}
\author{T.R.~Wyatt} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{Y.~Xie} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{R.~Yamada} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{S.~Yang} \affiliation{University of Science and Technology of China, Hefei, People's Republic of China}
\author{W.-C.~Yang} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{T.~Yasuda} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{Y.A.~Yatsunenko} \affiliation{Joint Institute for Nuclear Research, Dubna, Russia}
\author{W.~Ye} \affiliation{State University of New York, Stony Brook, New York 11794, USA}
\author{Z.~Ye} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{H.~Yin} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{K.~Yip} \affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{S.W.~Youn} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{J.M.~Yu} \affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\author{J.~Zennamo} \affiliation{State University of New York, Buffalo, New York 14260, USA}
\author{T.~Zhao} \affiliation{University of Washington, Seattle, Washington 98195, USA}
\author{T.G.~Zhao} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{B.~Zhou} \affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\author{J.~Zhu} \affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\author{M.~Zielinski} \affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{D.~Zieminska} \affiliation{Indiana University, Bloomington, Indiana 47405, USA}
\author{L.~Zivkovic} \affiliation{Brown University, Providence, Rhode Island 02912, USA}
%
% visitor_addresses.tex                       13 May 2012 
%  available symbols are:
%  $\ast, \dag, \ddag, \S, \P, $\|$, $\ast\ast$, \dag\dag, \ddag\ddag ,\#
%
\collaboration{The D0 Collaboration\footnote{with visitors from
%{alton}
$^{a}$Augustana College, Sioux Falls, SD, USA,
%{burdin}
$^{b}$The University of Liverpool, Liverpool, UK,
%{garcia-guerra}
$^{c}$UPIITA-IPN, Mexico City, Mexico,
%{grohsjean}
$^{d}$DESY, Hamburg, Germany,
,%{partridge}
$^{e}$SLAC, Menlo Park, CA, USA,
%{hesketh}
$^{f}$University College London, London, UK,
%{luna-garcia}
$^{g}$Centro de Investigacion en Computacion - IPN, Mexico City, Mexico,
%{podesta-lerma}
$^{h}$ECFM, Universidad Autonoma de Sinaloa, Culiac\'an, Mexico
and
%{santos}
$^{i}$Universidade Estadual Paulista, S\~ao Paulo, Brazil.
%{falkowski}
%$^{?}$Laboratoire de Physique Theorique, Orsay, FR,
%{hooper}
%$^{?}$Visitor from Bradley University, Peoria, IL, USA.
%{kozminski}
%$^{?}$}Visitor from Lewis University, Romeoville, IL, USA.
%{weber}
%$^{?}$Universit{\"a}t Bern, Bern, Switzerland.
%{deceased}
%$^{\ddag}$Deceased.
}} \noaffiliation
%
\vskip 0.25cm

